Hadamard-Pi: Equational Quantum Programming

Quantum computing offers advantages over classical computation, yet the precise features that set the two apart remain unclear. In the standard quantum circuit model, adding a 1-qubit basis-changing gate -- commonly chosen to be the Hadamard gate -- to a universal set of classical reversible gates yields computationally universal quantum computation. However, the computational behaviours enabled by this addition are not fully characterised. We give such a characterisation by introducing a small quantum programming language extending the universal classical reversible programming language $\Pi$ with a single primitive corresponding to the Hadamard gate. The language comes equipped with a sound and complete categorical semantics that is specified by a purely equational theory. Completeness is shown by means of a novel finite presentation, and a corresponding synthesis algorithm, for the groups of orthogonal matrices with entries in the ring $\mathbb{Z}[\tfrac{1}{\sqrt{2}}]$.

==> robustExternalize/robExt-01DF6418800934DB25D6B6AF8ADA80DA-out.tex <==
\def\robExtWidth{221.73358pt}\def\robExtHeight{27.80894pt}\def\robExtDepth{22.66895pt}


==> robustExternalize/robExt-020F16CBD7EEF2209D82590CE41EE860-out.tex <==
\def\robExtWidth{299.87155pt}\def\robExtHeight{34.3082pt}\def\robExtDepth{29.16821pt}


==> robustExternalize/robExt-031F4AC93E1A49EEBA0C0E1B47C38FA0-out.tex <==
\def\robExtWidth{214.23834pt}\def\robExtHeight{35.29906pt}\def\robExtDepth{30.15907pt}


==> robustExternalize/robExt-036944FFFB55E6DEF22D1EEB54EA30A5-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{22.93393pt}\def\robExtDepth{18.19394pt}


==> robustExternalize/robExt-04521885267F3F889A25E2C88B6D5EE5-out.tex <==
\def\robExtWidth{77.12044pt}\def\robExtHeight{16.6153pt}\def\robExtDepth{11.47533pt}


==> robustExternalize/robExt-045DDF3EDF7461E42EA98D434B0E0A9D-out.tex <==
\def\robExtWidth{129.80353pt}\def\robExtHeight{20.9174pt}\def\robExtDepth{15.37741pt}


==> robustExternalize/robExt-063B3766BD104AEFE38B128164D860AB-out.tex <==
\def\robExtWidth{228.47841pt}\def\robExtHeight{57.57454pt}\def\robExtDepth{52.43456pt}


==> robustExternalize/robExt-0678648532AA46B1E556C49E7D11B0BB-out.tex <==
\def\robExtWidth{180.75555pt}\def\robExtHeight{63.7259pt}\def\robExtDepth{58.58592pt}


==> robustExternalize/robExt-070D55DC7132B1EED000D3A73CFCB849-out.tex <==
\def\robExtWidth{57.28558pt}\def\robExtHeight{22.58643pt}\def\robExtDepth{17.44644pt}


==> robustExternalize/robExt-0745EF80D528001019929549001D9233-out.tex <==
\def\robExtWidth{127.84485pt}\def\robExtHeight{37.20981pt}\def\robExtDepth{32.06981pt}


==> robustExternalize/robExt-0855BBEF7E0A3D10DBEE078ADA401A30-out.tex <==
\def\robExtWidth{105.71553pt}\def\robExtHeight{25.25584pt}\def\robExtDepth{20.11584pt}


==> robustExternalize/robExt-096C653BE1184A38DDE339716CDD4CE8-out.tex <==
\def\robExtWidth{101.59418pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-0A6B02B54165CC518AE3F5C1F68C2EB7-out.tex <==
\def\robExtWidth{197.77689pt}\def\robExtHeight{26.23335pt}\def\robExtDepth{21.09335pt}


==> robustExternalize/robExt-0AA163DCDB6C1B2C554A14D00ADA8041-out.tex <==
\def\robExtWidth{146.23851pt}\def\robExtHeight{16.74208pt}\def\robExtDepth{11.6021pt}


==> robustExternalize/robExt-0C04676178B290C47C2FC68C72D8AFC5-out.tex <==
\def\robExtWidth{159.98137pt}\def\robExtHeight{32.74596pt}\def\robExtDepth{27.60597pt}


==> robustExternalize/robExt-0CBCB996A95FAE9AE80909FDB083ED69-out.tex <==
\def\robExtWidth{165.0164pt}\def\robExtHeight{33.72346pt}\def\robExtDepth{28.58348pt}


==> robustExternalize/robExt-0D382BC6CEEF37E8ED33F69B046A7F9F-out.tex <==
\def\robExtWidth{159.98137pt}\def\robExtHeight{40.23608pt}\def\robExtDepth{35.09608pt}


==> robustExternalize/robExt-0DDB5F8DD6153D9B2361CC3BD1DDADB0-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{24.82684pt}\def\robExtDepth{20.08685pt}


==> robustExternalize/robExt-0F8F6253A5230A409C798B829B0DC3A8-out.tex <==
\def\robExtWidth{135.09517pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-0FD120C5107D0E96B5920E9ADFEC5AC3-out.tex <==
\def\robExtWidth{82.15547pt}\def\robExtHeight{29.4032pt}\def\robExtDepth{24.26321pt}


==> robustExternalize/robExt-10D29AF707BBE22AE02F9FCCBE69EEEF-out.tex <==
\def\robExtWidth{161.64644pt}\def\robExtHeight{43.2548pt}\def\robExtDepth{38.1148pt}


==> robustExternalize/robExt-12AA5789F2D96BFF8A6C251DBE7C566A-out.tex <==
\def\robExtWidth{94.70929pt}\def\robExtHeight{12.8389pt}\def\robExtDepth{7.69891pt}


==> robustExternalize/robExt-12DE0970B7D0385A1E98DC62DC51C85E-out.tex <==
\def\robExtWidth{135.09517pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-1364E3FB816B98718FDE24EBB1602DB8-out.tex <==
\def\robExtWidth{127.15408pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-15D77DEF4021A347F2888C81B5A32C43-out.tex <==
\def\robExtWidth{113.25566pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-16993EDA72AE17F9E5B13B760E3E6F6A-out.tex <==
\def\robExtWidth{82.75177pt}\def\robExtHeight{35.28287pt}\def\robExtDepth{30.14288pt}


==> robustExternalize/robExt-1752BCC720121650F9AEF285FEC1E716-out.tex <==
\def\robExtWidth{106.72734pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-1A62282AFF5D2B446B41B37A4D79282C-out.tex <==
\def\robExtWidth{30.20703pt}\def\robExtHeight{17.05032pt}\def\robExtDepth{11.51033pt}


==> robustExternalize/robExt-1D3C2AEEB8A92671EAFE6E0F8012CD79-out.tex <==
\def\robExtWidth{65.69391pt}\def\robExtHeight{28.00558pt}\def\robExtDepth{23.2656pt}


==> robustExternalize/robExt-1F9CFC992E6F16621B35B6359E514952-out.tex <==
\def\robExtWidth{129.80353pt}\def\robExtHeight{22.46948pt}\def\robExtDepth{17.32948pt}


==> robustExternalize/robExt-2223F5A22BFEACAA23B63BAD79BD67D0-out.tex <==
\def\robExtWidth{111.23294pt}\def\robExtHeight{14.42296pt}\def\robExtDepth{9.28297pt}


==> robustExternalize/robExt-252186A7352C6DC6475089DC10DA93DE-out.tex <==
\def\robExtWidth{110.623pt}\def\robExtHeight{25.86975pt}\def\robExtDepth{20.32977pt}


==> robustExternalize/robExt-263E31F0B9430DADACEA4FE112F3FAE8-out.tex <==
\def\robExtWidth{108.06082pt}\def\robExtHeight{20.30113pt}\def\robExtDepth{15.56116pt}


==> robustExternalize/robExt-26CAEFF2E5F4EF4E2E3B9F068993911A-out.tex <==
\def\robExtWidth{65.8931pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-27A763C31FADA8BCEDB34A922D33EAA3-out.tex <==
\def\robExtWidth{140.16258pt}\def\robExtHeight{40.73622pt}\def\robExtDepth{38.5292pt}


==> robustExternalize/robExt-27BF5BE4834C52A99F6BF1D5FA931CF5-out.tex <==
\def\robExtWidth{58.54886pt}\def\robExtHeight{30.20721pt}\def\robExtDepth{25.06725pt}


==> robustExternalize/robExt-280B51E5FBB59828338B19705B263399-out.tex <==
\def\robExtWidth{177.65215pt}\def\robExtHeight{38.95305pt}\def\robExtDepth{33.81305pt}


==> robustExternalize/robExt-2895F1B82026859B25915B51CFBC66B7-out.tex <==
\def\robExtWidth{101.99036pt}\def\robExtHeight{22.62009pt}\def\robExtDepth{17.48012pt}


==> robustExternalize/robExt-2973BC6906DE56CF44297ABB7488AFEC-out.tex <==
\def\robExtWidth{135.64516pt}\def\robExtHeight{46.82935pt}\def\robExtDepth{41.68935pt}


==> robustExternalize/robExt-2A3D296F86927CB862CBA4E5D06D5F19-out.tex <==
\def\robExtWidth{125.6284pt}\def\robExtHeight{44.6087pt}\def\robExtDepth{39.4687pt}


==> robustExternalize/robExt-2CB781338B985B48C2131D659D9AF81F-out.tex <==
\def\robExtWidth{68.3861pt}\def\robExtHeight{16.65031pt}\def\robExtDepth{11.91034pt}


==> robustExternalize/robExt-2D7A32BE4278AD65894C787B02596394-out.tex <==
\def\robExtWidth{94.95596pt}\def\robExtHeight{28.38347pt}\def\robExtDepth{23.24348pt}


==> robustExternalize/robExt-2ED9739C431627A86AE2E5FA6EC4A22E-out.tex <==
\def\robExtWidth{135.09517pt}\def\robExtHeight{46.82935pt}\def\robExtDepth{41.68935pt}


==> robustExternalize/robExt-2F652AAC9721FE449DE476F6B4968E01-out.tex <==
\def\robExtWidth{115.4777pt}\def\robExtHeight{27.80894pt}\def\robExtDepth{22.66895pt}


==> robustExternalize/robExt-31633B890879384C8541C4D90745AD44-out.tex <==
\def\robExtWidth{130.9924pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-31A67D323A3E7E114BE16C139D1F2A4A-out.tex <==
\def\robExtWidth{165.8007pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-333D894A8DD1ABF05D5C9A566EB34BD7-out.tex <==
\def\robExtWidth{77.12044pt}\def\robExtHeight{24.10542pt}\def\robExtDepth{18.96544pt}


==> robustExternalize/robExt-3347AD5ABDEE05E60819C8B7C75A010D-out.tex <==
\def\robExtWidth{75.0108pt}\def\robExtHeight{20.30113pt}\def\robExtDepth{15.56116pt}


==> robustExternalize/robExt-3508D6587D8F077B9CA6E0BDC49C3E13-out.tex <==
\def\robExtWidth{91.24539pt}\def\robExtHeight{40.27585pt}\def\robExtDepth{35.13585pt}


==> robustExternalize/robExt-35DBFB0E1E28CA279EAEC106C07E1BEE-out.tex <==
\def\robExtWidth{135.64516pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-36400A197666B45C66B6C6139C82FEC4-out.tex <==
\def\robExtWidth{141.1846pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-36EF22745943D672D4FBA19B63798A71-out.tex <==
\def\robExtWidth{65.8931pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-379372CB82B23E7C568C7079CFAFD995-out.tex <==
\def\robExtWidth{122.89967pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-38AA4228FC14C08B78D57E43DE76BE88-out.tex <==
\def\robExtWidth{89.59427pt}\def\robExtHeight{26.67847pt}\def\robExtDepth{21.53848pt}


==> robustExternalize/robExt-39594126D4C993D9B00E56DA3ED26D2F-out.tex <==
\def\robExtWidth{83.16031pt}\def\robExtHeight{21.13821pt}\def\robExtDepth{15.99825pt}


==> robustExternalize/robExt-3BC4057373A941282E7A15D3337D42D4-out.tex <==
\def\robExtWidth{84.55914pt}\def\robExtHeight{21.15321pt}\def\robExtDepth{16.01321pt}


==> robustExternalize/robExt-3C48E7844FA51B83463E291B8B158E79-out.tex <==
\def\robExtWidth{99.56651pt}\def\robExtHeight{33.65527pt}\def\robExtDepth{28.51527pt}


==> robustExternalize/robExt-3DD56FF95D17A2A0217AA922691CB10D-out.tex <==
\def\robExtWidth{298.90913pt}\def\robExtHeight{62.12047pt}\def\robExtDepth{56.98048pt}


==> robustExternalize/robExt-3E6DB63E3BCFBC86D96E91D74A6BE73F-out.tex <==
\def\robExtWidth{109.5655pt}\def\robExtHeight{38.04373pt}\def\robExtDepth{32.90375pt}


==> robustExternalize/robExt-3F4151DA386B3F20A19A1BBB8D1176DD-out.tex <==
\def\robExtWidth{137.60637pt}\def\robExtHeight{29.4032pt}\def\robExtDepth{24.26321pt}


==> robustExternalize/robExt-3F55C8A3B5FFDE697640F76B4E89DD9B-out.tex <==
\def\robExtWidth{68.56808pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-40067E30F2105E99944A50FF32FD2F14-out.tex <==
\def\robExtWidth{135.09517pt}\def\robExtHeight{46.82935pt}\def\robExtDepth{41.68935pt}


==> robustExternalize/robExt-401A6E0FB7DF86C5BF28CA77F8CA18C2-out.tex <==
\def\robExtWidth{208.06982pt}\def\robExtHeight{31.28891pt}\def\robExtDepth{25.74893pt}


==> robustExternalize/robExt-407B870AD78D4AFE7F1EC40D1758553D-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{22.93393pt}\def\robExtDepth{18.19394pt}


==> robustExternalize/robExt-40EC9B141DAB6DF4BB9FC0A987471EDF-out.tex <==
\def\robExtWidth{221.4941pt}\def\robExtHeight{58.65022pt}\def\robExtDepth{53.51024pt}


==> robustExternalize/robExt-41763D8A2E1CDC0EC44DD1CA59A6D6C8-out.tex <==
\def\robExtWidth{140.16258pt}\def\robExtHeight{40.73622pt}\def\robExtDepth{38.5292pt}


==> robustExternalize/robExt-41CDBE059ABD49CEEA3A71099C67D8A3-out.tex <==
\def\robExtWidth{29.4281pt}\def\robExtHeight{16.74825pt}\def\robExtDepth{11.60825pt}


==> robustExternalize/robExt-429956949367BB92179B763CB87EBE18-out.tex <==
\def\robExtWidth{187.3914pt}\def\robExtHeight{40.23608pt}\def\robExtDepth{35.09608pt}


==> robustExternalize/robExt-431B7F6369B699042846C237918246E8-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{17.98158pt}\def\robExtDepth{13.24158pt}


==> robustExternalize/robExt-43563C4F6915C3D0F6EC12273E0F4583-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{22.46947pt}\def\robExtDepth{17.3295pt}


==> robustExternalize/robExt-43BD10DAB7FD38FBE0625B0823682EF3-out.tex <==
\def\robExtWidth{99.8508pt}\def\robExtHeight{38.13419pt}\def\robExtDepth{32.99419pt}


==> robustExternalize/robExt-43FFE41B18A2326051FE1F32778068C5-out.tex <==
\def\robExtWidth{99.8508pt}\def\robExtHeight{31.28891pt}\def\robExtDepth{26.14893pt}


==> robustExternalize/robExt-44EBE2DD039DA0AFD36DCEC0BD22BDDA-out.tex <==
\def\robExtWidth{188.00734pt}\def\robExtHeight{62.12047pt}\def\robExtDepth{56.98048pt}


==> robustExternalize/robExt-46061372E232E07E56C00C50D27B25EB-out.tex <==
\def\robExtWidth{41.5881pt}\def\robExtHeight{16.65031pt}\def\robExtDepth{11.91034pt}


==> robustExternalize/robExt-460AE5FCE845224DB31D6D9BA50CB016-out.tex <==
\def\robExtWidth{155.8606pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-471AA43F629A581F5A9BB56AC0DC9296-out.tex <==
\def\robExtWidth{79.74187pt}\def\robExtHeight{18.54439pt}\def\robExtDepth{13.80438pt}


==> robustExternalize/robExt-47C63C63320DF18FAA6CF37971F27501-out.tex <==
\def\robExtWidth{201.40979pt}\def\robExtHeight{29.90068pt}\def\robExtDepth{24.7607pt}


==> robustExternalize/robExt-4A0926D747DFB985EA8416B983E27E54-out.tex <==
\def\robExtWidth{242.52281pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-4C11D86849384E6F597101705940BDDC-out.tex <==
\def\robExtWidth{70.8491pt}\def\robExtHeight{19.4535pt}\def\robExtDepth{14.71353pt}


==> robustExternalize/robExt-4C5EF3420E3D68175669C6FB81BAD6A4-out.tex <==
\def\robExtWidth{137.60637pt}\def\robExtHeight{29.4032pt}\def\robExtDepth{24.26321pt}


==> robustExternalize/robExt-4C6B752577E15F435F8E16FA0C74BC44-out.tex <==
\def\robExtWidth{161.64644pt}\def\robExtHeight{43.2548pt}\def\robExtDepth{38.1148pt}


==> robustExternalize/robExt-4D311FCB7EFDAACD03657F8D3328C07D-out.tex <==
\def\robExtWidth{180.75555pt}\def\robExtHeight{62.65022pt}\def\robExtDepth{57.51024pt}


==> robustExternalize/robExt-4D75AE38E7F2ECCB74159067D2C27DE2-out.tex <==
\def\robExtWidth{33.05061pt}\def\robExtHeight{16.6153pt}\def\robExtDepth{11.47533pt}


==> robustExternalize/robExt-4DE0F304A28DA70A1CB6C929F9726A5C-out.tex <==
\def\robExtWidth{289.0032pt}\def\robExtHeight{31.8557pt}\def\robExtDepth{26.71571pt}


==> robustExternalize/robExt-5018BC30145C8E8320D0703708F3B3EA-out.tex <==
\def\robExtWidth{138.8552pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-509420ED681C0E21BD021BFC83392648-out.tex <==
\def\robExtWidth{135.09714pt}\def\robExtHeight{26.67847pt}\def\robExtDepth{21.53848pt}


==> robustExternalize/robExt-51A649C2BA3C0A85D1051095ABC55BCA-out.tex <==
\def\robExtWidth{131.9405pt}\def\robExtHeight{25.25584pt}\def\robExtDepth{20.11584pt}


==> robustExternalize/robExt-53C8183424A9B5AA0A37830149BA99E4-out.tex <==
\def\robExtWidth{161.64644pt}\def\robExtHeight{43.2548pt}\def\robExtDepth{38.1148pt}


==> robustExternalize/robExt-55EF85B571CB0F9973B0FABE9DA205AF-out.tex <==
\def\robExtWidth{57.28558pt}\def\robExtHeight{17.63408pt}\def\robExtDepth{12.49408pt}


==> robustExternalize/robExt-58A427318F2B5F3C83DE9A411F918485-out.tex <==
\def\robExtWidth{149.99599pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-58E29496F48CCBC8A9E11960754EA9B2-out.tex <==
\def\robExtWidth{165.8007pt}\def\robExtHeight{30.646pt}\def\robExtDepth{25.50601pt}


==> robustExternalize/robExt-5DD878B2D49B3E19DFC21E4384F665A0-out.tex <==
\def\robExtWidth{149.39015pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-5E452EF5F1F82178CDD98F2A21F404D8-out.tex <==
\def\robExtWidth{162.08342pt}\def\robExtHeight{37.99138pt}\def\robExtDepth{32.85138pt}


==> robustExternalize/robExt-5E8734658AE499B662854B78EA3829A5-out.tex <==
\def\robExtWidth{201.40979pt}\def\robExtHeight{29.90068pt}\def\robExtDepth{24.7607pt}


==> robustExternalize/robExt-5E9D3CD2087FFEE05FEB7F929626412F-out.tex <==
\def\robExtWidth{57.28558pt}\def\robExtHeight{22.58643pt}\def\robExtDepth{17.44644pt}


==> robustExternalize/robExt-5EA7293F243CD30E71B1AEF0E470D6E3-out.tex <==
\def\robExtWidth{77.12044pt}\def\robExtHeight{24.10542pt}\def\robExtDepth{18.96544pt}


==> robustExternalize/robExt-60A3DFB04F9C957C4BA6BA3F25831460-out.tex <==
\def\robExtWidth{207.25879pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-6400CC871BE2DE5FDC31C56F86ACCA71-out.tex <==
\def\robExtWidth{135.09517pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-65FB661FF4B5100E988D3204C8549C9A-out.tex <==
\def\robExtWidth{180.75555pt}\def\robExtHeight{62.65022pt}\def\robExtDepth{57.51024pt}


==> robustExternalize/robExt-67AAF3467F8D0D539E0C739226B1A8D9-out.tex <==
\def\robExtWidth{50.71754pt}\def\robExtHeight{22.93393pt}\def\robExtDepth{17.79395pt}


==> robustExternalize/robExt-69F4AC7EFA747F43920E47451051F43E-out.tex <==
\def\robExtWidth{170.25093pt}\def\robExtHeight{34.3082pt}\def\robExtDepth{29.16821pt}


==> robustExternalize/robExt-6B34FA2525B04CB640C494F86D6B76C3-out.tex <==
\def\robExtWidth{77.12044pt}\def\robExtHeight{24.10542pt}\def\robExtDepth{18.96544pt}


==> robustExternalize/robExt-6BAC0C849B9B26FA5122488DE52B43A2-out.tex <==
\def\robExtWidth{35.88255pt}\def\robExtHeight{16.65782pt}\def\robExtDepth{11.91782pt}


==> robustExternalize/robExt-6EC26500859CDA2BCB78B050BDC5C7FC-out.tex <==
\def\robExtWidth{161.64644pt}\def\robExtHeight{43.2548pt}\def\robExtDepth{38.1148pt}


==> robustExternalize/robExt-6ED71A7880CE1480ED3FABA10C997749-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-6F4B0F0A47B01DC1626112EB3B9E8628-out.tex <==
\def\robExtWidth{217.58685pt}\def\robExtHeight{31.8557pt}\def\robExtDepth{26.71571pt}


==> robustExternalize/robExt-6F7A6F4F31B9AEC625821106B61B0889-out.tex <==
\def\robExtWidth{101.59418pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-6FF4301951575949AFBD9729C20A5DFB-out.tex <==
\def\robExtWidth{146.62018pt}\def\robExtHeight{41.01752pt}\def\robExtDepth{35.87752pt}


==> robustExternalize/robExt-70395A80D6C79F2D50EAF99973027AC8-out.tex <==
\def\robExtWidth{135.64516pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-707F854CFEC99697108CF50F9B80D8CA-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{22.93393pt}\def\robExtDepth{17.79395pt}


==> robustExternalize/robExt-7218EF42E4E4268F658768792D179761-out.tex <==
\def\robExtWidth{353.84306pt}\def\robExtHeight{35.28287pt}\def\robExtDepth{30.14288pt}


==> robustExternalize/robExt-74AB5BFE374184735283342A498B6860-out.tex <==
\def\robExtWidth{131.9405pt}\def\robExtHeight{48.87662pt}\def\robExtDepth{43.73662pt}


==> robustExternalize/robExt-7545599422B7D8822A74110F658C117D-out.tex <==
\def\robExtWidth{159.98137pt}\def\robExtHeight{32.74596pt}\def\robExtDepth{27.60597pt}


==> robustExternalize/robExt-76F8D26708B41D0F671A7EAC28F6B25A-out.tex <==
\def\robExtWidth{187.3914pt}\def\robExtHeight{40.23608pt}\def\robExtDepth{35.09608pt}


==> robustExternalize/robExt-776B3D6EE6D4A34AD5AB9E853954EEB6-out.tex <==
\def\robExtWidth{35.7945pt}\def\robExtHeight{40.27585pt}\def\robExtDepth{35.13585pt}


==> robustExternalize/robExt-7802110B9175F12AD635F4F55DB247C3-out.tex <==
\def\robExtWidth{102.21468pt}\def\robExtHeight{22.58643pt}\def\robExtDepth{17.44644pt}


==> robustExternalize/robExt-78F76AB6E56396F3BA88A558564129CB-out.tex <==
\def\robExtWidth{188.00734pt}\def\robExtHeight{62.12047pt}\def\robExtDepth{56.98048pt}


==> robustExternalize/robExt-79EA5626452C0076CEB498B09878BD40-out.tex <==
\def\robExtWidth{57.28558pt}\def\robExtHeight{22.58643pt}\def\robExtDepth{17.44644pt}


==> robustExternalize/robExt-79F0AD6BCF25964A1DE649F581810C07-out.tex <==
\def\robExtWidth{169.25131pt}\def\robExtHeight{38.95305pt}\def\robExtDepth{33.81305pt}


==> robustExternalize/robExt-7AF206DEBD596EA82C9A0AC160FB3339-out.tex <==
\def\robExtWidth{159.75626pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-7CAE78B13B990846AF253347364D9337-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{22.93393pt}\def\robExtDepth{17.79395pt}


==> robustExternalize/robExt-7D35786717765AF2B711742EED6A4C36-out.tex <==
\def\robExtWidth{99.8508pt}\def\robExtHeight{31.28891pt}\def\robExtDepth{26.14893pt}


==> robustExternalize/robExt-7EC268DD0E7E30156AFF05402A9C9DC4-out.tex <==
\def\robExtWidth{142.6414pt}\def\robExtHeight{21.91309pt}\def\robExtDepth{16.77309pt}


==> robustExternalize/robExt-7FB21DFF2EB2C0C44DA3F01C2B89C6C8-out.tex <==
\def\robExtWidth{109.5655pt}\def\robExtHeight{26.23335pt}\def\robExtDepth{21.09335pt}


==> robustExternalize/robExt-7FD2987D66A3DEEBD99543EBFC519386-out.tex <==
\def\robExtWidth{77.12044pt}\def\robExtHeight{31.59554pt}\def\robExtDepth{26.45557pt}


==> robustExternalize/robExt-8017BD26C630B137DD23694FC68E33B9-out.tex <==
\def\robExtWidth{61.48975pt}\def\robExtHeight{27.76266pt}\def\robExtDepth{22.62268pt}


==> robustExternalize/robExt-8165DDF478DFC849C56621C4E5F72BFD-out.tex <==
\def\robExtWidth{104.36774pt}\def\robExtHeight{21.13821pt}\def\robExtDepth{15.99825pt}


==> robustExternalize/robExt-8370CECA198BE460CDD3533D8E88DD31-out.tex <==
\def\robExtWidth{142.6414pt}\def\robExtHeight{21.91309pt}\def\robExtDepth{16.77309pt}


==> robustExternalize/robExt-8488F40B2E39C4BA04A581C1B5C7CBFC-out.tex <==
\def\robExtWidth{128.68774pt}\def\robExtHeight{26.09058pt}\def\robExtDepth{20.5506pt}


==> robustExternalize/robExt-8502F580A47748D6D336AE12AAA6B22C-out.tex <==
\def\robExtWidth{158.78745pt}\def\robExtHeight{35.29906pt}\def\robExtDepth{30.15907pt}


==> robustExternalize/robExt-858B17406C8DFEE168077C20499A8534-out.tex <==
\def\robExtWidth{114.84021pt}\def\robExtHeight{42.77104pt}\def\robExtDepth{37.63107pt}


==> robustExternalize/robExt-8706B2BAADAA7CC560E2356A88C4DDDD-out.tex <==
\def\robExtWidth{139.22752pt}\def\robExtHeight{18.20445pt}\def\robExtDepth{13.46448pt}


==> robustExternalize/robExt-896892E4FF3C53B372A1C5D860829FEA-out.tex <==
\def\robExtWidth{136.19514pt}\def\robExtHeight{46.82935pt}\def\robExtDepth{41.68935pt}


==> robustExternalize/robExt-89D3F6E8C408B28489634032D219919E-out.tex <==
\def\robExtWidth{152.31071pt}\def\robExtHeight{34.17224pt}\def\robExtDepth{29.03226pt}


==> robustExternalize/robExt-8AD3D3A0D4A79E7AA5FC80EDA602A4D5-out.tex <==
\def\robExtWidth{137.60637pt}\def\robExtHeight{21.91309pt}\def\robExtDepth{16.77309pt}


==> robustExternalize/robExt-8B7D5D1481C6B0035647C0D74850EDC3-out.tex <==
\def\robExtWidth{298.90913pt}\def\robExtHeight{62.12047pt}\def\robExtDepth{56.98048pt}


==> robustExternalize/robExt-8BD4527B0E51B8DB9F41187382693510-out.tex <==
\def\robExtWidth{176.2702pt}\def\robExtHeight{19.4535pt}\def\robExtDepth{14.71353pt}


==> robustExternalize/robExt-8C28BF0B7C4276A41D0F0939A4DC0CC6-out.tex <==
\def\robExtWidth{282.63553pt}\def\robExtHeight{58.65022pt}\def\robExtDepth{53.51024pt}


==> robustExternalize/robExt-8F00BEB5FE0BFC586D6286DF91AC47C6-out.tex <==
\def\robExtWidth{169.25131pt}\def\robExtHeight{38.95305pt}\def\robExtDepth{33.81305pt}


==> robustExternalize/robExt-9024E7827E2F3491F51F0BB8656E4AAC-out.tex <==
\def\robExtWidth{72.3636pt}\def\robExtHeight{21.14572pt}\def\robExtDepth{16.00572pt}


==> robustExternalize/robExt-907BC573BEC9271B744A2690492CE46D-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{18.38158pt}\def\robExtDepth{12.84158pt}


==> robustExternalize/robExt-912C5CE865C2F745098E7D6A3718F92C-out.tex <==
\def\robExtWidth{53.74811pt}\def\robExtHeight{21.13821pt}\def\robExtDepth{15.99825pt}


==> robustExternalize/robExt-918E1144F5A06D57727A7FAF45FE8437-out.tex <==
\def\robExtWidth{142.54558pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-94796D2B052A6023F85712824E8D546A-out.tex <==
\def\robExtWidth{39.50507pt}\def\robExtHeight{28.38347pt}\def\robExtDepth{23.24348pt}


==> robustExternalize/robExt-95B330FCD468846C18BE30594D42C861-out.tex <==
\def\robExtWidth{87.1905pt}\def\robExtHeight{27.21086pt}\def\robExtDepth{22.07086pt}


==> robustExternalize/robExt-960FDD4F90FBFF664033BD6AF0B9FD0B-out.tex <==
\def\robExtWidth{87.1905pt}\def\robExtHeight{27.21086pt}\def\robExtDepth{22.07086pt}


==> robustExternalize/robExt-98890126230E91DBF5B026D838FC0420-out.tex <==
\def\robExtWidth{82.15547pt}\def\robExtHeight{29.4032pt}\def\robExtDepth{24.26321pt}


==> robustExternalize/robExt-9AB637C64E5B5E16C81A48E2EEE03449-out.tex <==
\def\robExtWidth{172.36874pt}\def\robExtHeight{31.50974pt}\def\robExtDepth{26.36975pt}


==> robustExternalize/robExt-9BA74289BBDCAEB182F381C87FA0EA7D-out.tex <==
\def\robExtWidth{82.67485pt}\def\robExtHeight{18.54439pt}\def\robExtDepth{13.80438pt}


==> robustExternalize/robExt-9C2734FB1FC4772F2A74E991D72291EE-out.tex <==
\def\robExtWidth{208.8498pt}\def\robExtHeight{31.28891pt}\def\robExtDepth{25.74893pt}


==> robustExternalize/robExt-9C3071395C6570453EB52E03CA51AF98-out.tex <==
\def\robExtWidth{221.73358pt}\def\robExtHeight{27.80894pt}\def\robExtDepth{22.66895pt}


==> robustExternalize/robExt-9D780009AC0A325D85A1EC759578C945-out.tex <==
\def\robExtWidth{135.64516pt}\def\robExtHeight{46.82935pt}\def\robExtDepth{41.68935pt}


==> robustExternalize/robExt-9D9C80BA198F09C56002A8BA77EBD78A-out.tex <==
\def\robExtWidth{176.56633pt}\def\robExtHeight{47.48888pt}\def\robExtDepth{42.34888pt}


==> robustExternalize/robExt-9E2D191ECC52FE1A711192FA21A710A3-out.tex <==
\def\robExtWidth{207.25879pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-A330BCAC15554D9D3598DA1F05E14606-out.tex <==
\def\robExtWidth{112.34688pt}\def\robExtHeight{16.65782pt}\def\robExtDepth{11.91782pt}


==> robustExternalize/robExt-A5D27C78589FE90E0F76C4552BD2E943-out.tex <==
\def\robExtWidth{35.7945pt}\def\robExtHeight{40.27585pt}\def\robExtDepth{35.13585pt}


==> robustExternalize/robExt-A5E7D1A1E6EB583BC5E054E52A9BBE5A-out.tex <==
\def\robExtWidth{211.9714pt}\def\robExtHeight{27.80894pt}\def\robExtDepth{22.66895pt}


==> robustExternalize/robExt-A604016B1C5FC45616A94686E4E7C99C-out.tex <==
\def\robExtWidth{135.64516pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-A6275D95EB976F610B26F11445A6F3C5-out.tex <==
\def\robExtWidth{115.2037pt}\def\robExtHeight{18.20445pt}\def\robExtDepth{13.46448pt}


==> robustExternalize/robExt-A819F712DEF1C45E5847BB4634F4E538-out.tex <==
\def\robExtWidth{125.6284pt}\def\robExtHeight{37.06622pt}\def\robExtDepth{31.92622pt}


==> robustExternalize/robExt-A87B969E5CBFD6052B420C3C2049ACE1-out.tex <==
\def\robExtWidth{159.98137pt}\def\robExtHeight{32.74596pt}\def\robExtDepth{27.60597pt}


==> robustExternalize/robExt-A8C84A87FA114B3113190D5AE7A71E65-out.tex <==
\def\robExtWidth{142.54558pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-A93168536C2AE70E36AE1D8B56AC5092-out.tex <==
\def\robExtWidth{158.33864pt}\def\robExtHeight{33.79166pt}\def\robExtDepth{28.65166pt}


==> robustExternalize/robExt-A98F4B1C2AC78477333CD1FC78A9673F-out.tex <==
\def\robExtWidth{149.99599pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-A9CA1B32BEFBDE0FCD585F769874CE53-out.tex <==
\def\robExtWidth{87.24916pt}\def\robExtHeight{37.06622pt}\def\robExtDepth{31.92622pt}


==> robustExternalize/robExt-AC8E97780B327D1D0A642FEE8853C6EE-out.tex <==
\def\robExtWidth{135.49406pt}\def\robExtHeight{31.28891pt}\def\robExtDepth{26.14893pt}


==> robustExternalize/robExt-AE771031643E14DF04EC9DDF90CB19FB-out.tex <==
\def\robExtWidth{131.9405pt}\def\robExtHeight{48.87662pt}\def\robExtDepth{43.73662pt}


==> robustExternalize/robExt-B0C5F3C71EE664DAEEF882AEC837508C-out.tex <==
\def\robExtWidth{193.28165pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-B0EA402E04BCB75178DAE56E3732F93D-out.tex <==
\def\robExtWidth{18.04703pt}\def\robExtHeight{20.12933pt}\def\robExtDepth{14.98935pt}


==> robustExternalize/robExt-B19C0B748D53CF00579B412B283FDB0A-out.tex <==
\def\robExtWidth{159.98137pt}\def\robExtHeight{40.23608pt}\def\robExtDepth{35.09608pt}


==> robustExternalize/robExt-B28B1746DF16072D07D87C5AAE78FC88-out.tex <==
\def\robExtWidth{126.53416pt}\def\robExtHeight{18.54439pt}\def\robExtDepth{13.80438pt}


==> robustExternalize/robExt-B4ACF69F49F95FF1C77E0329DDB17E50-out.tex <==
\def\robExtWidth{41.267pt}\def\robExtHeight{26.67847pt}\def\robExtDepth{21.53848pt}


==> robustExternalize/robExt-B571AA1D5CA53C10BD9C53FE3491C4E8-out.tex <==
\def\robExtWidth{30.19202pt}\def\robExtHeight{16.65782pt}\def\robExtDepth{11.91782pt}


==> robustExternalize/robExt-BAD44F5BA25D03ED5A05B6C72BB91219-out.tex <==
\def\robExtWidth{84.55914pt}\def\robExtHeight{21.15321pt}\def\robExtDepth{16.01321pt}


==> robustExternalize/robExt-BB9011E443AB4AA1794D5BA912A1CD01-out.tex <==
\def\robExtWidth{129.80353pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-BDE9D165F6057B3AE33247447D21D3C8-out.tex <==
\def\robExtWidth{104.53047pt}\def\robExtHeight{40.23607pt}\def\robExtDepth{35.0961pt}


==> robustExternalize/robExt-BE3ECFC373E9461A50C6EC4E3DD9B699-out.tex <==
\def\robExtWidth{193.28165pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-BE62AC58F028899EA833F6010A254013-out.tex <==
\def\robExtWidth{104.53047pt}\def\robExtHeight{40.23607pt}\def\robExtDepth{35.0961pt}


==> robustExternalize/robExt-BEEE6580DFDC7524F90C77F7874AB7ED-out.tex <==
\def\robExtWidth{243.45824pt}\def\robExtHeight{62.12047pt}\def\robExtDepth{56.98048pt}


==> robustExternalize/robExt-BF4F7E6877FE172F43A9F10615232D13-out.tex <==
\def\robExtWidth{147.5086pt}\def\robExtHeight{24.91135pt}\def\robExtDepth{19.77138pt}


==> robustExternalize/robExt-BF6B77AF1E5AF844BE29BB93AD215A22-out.tex <==
\def\robExtWidth{138.7727pt}\def\robExtHeight{24.04272pt}\def\robExtDepth{18.90276pt}


==> robustExternalize/robExt-BFC5A32F884300454C084F5CF18ACCBA-out.tex <==
\def\robExtWidth{61.48975pt}\def\robExtHeight{25.86975pt}\def\robExtDepth{20.32977pt}


==> robustExternalize/robExt-C1C764CEF594FCB01D13EDB9C3CD27DE-out.tex <==
\def\robExtWidth{181.01828pt}\def\robExtHeight{35.28287pt}\def\robExtDepth{30.14288pt}


==> robustExternalize/robExt-C2574D6D64C14F54CFD6D4CDE5B7F926-out.tex <==
\def\robExtWidth{61.48975pt}\def\robExtHeight{25.86975pt}\def\robExtDepth{20.32977pt}


==> robustExternalize/robExt-C28283303C8F444E327C7D6C412DD303-out.tex <==
\def\robExtWidth{243.45824pt}\def\robExtHeight{62.12047pt}\def\robExtDepth{56.98048pt}


==> robustExternalize/robExt-C361410718E93681110771EC425BDB16-out.tex <==
\def\robExtWidth{211.9714pt}\def\robExtHeight{27.80894pt}\def\robExtDepth{22.66895pt}


==> robustExternalize/robExt-C40F14952769F39179C41B7A3BB571C2-out.tex <==
\def\robExtWidth{54.79138pt}\def\robExtHeight{15.92114pt}\def\robExtDepth{10.78116pt}


==> robustExternalize/robExt-C4189FFA4D2389056167BDA22E1623D4-out.tex <==
\def\robExtWidth{49.77754pt}\def\robExtHeight{22.46948pt}\def\robExtDepth{17.32948pt}


==> robustExternalize/robExt-C467F106866F62E3CCD1E30109BFFDF5-out.tex <==
\def\robExtWidth{99.56651pt}\def\robExtHeight{33.65527pt}\def\robExtDepth{28.51527pt}


==> robustExternalize/robExt-C7FC6ECEE53AA80516879F06E9B40DA1-out.tex <==
\def\robExtWidth{129.80353pt}\def\robExtHeight{20.9174pt}\def\robExtDepth{15.37741pt}


==> robustExternalize/robExt-CA099BDA6705B71E5E5415023CEB05FA-out.tex <==
\def\robExtWidth{182.25687pt}\def\robExtHeight{47.48888pt}\def\robExtDepth{42.34888pt}


==> robustExternalize/robExt-CC6BDFC910FEF6A604E744DC7F77769D-out.tex <==
\def\robExtWidth{106.72734pt}\def\robExtHeight{23.80074pt}\def\robExtDepth{18.66074pt}


==> robustExternalize/robExt-CCA46ACDB2B25A43547761926CA01057-out.tex <==
\def\robExtWidth{66.27905pt}\def\robExtHeight{24.04272pt}\def\robExtDepth{18.90276pt}


==> robustExternalize/robExt-CD531E960C5B43FCEA9ECC8D24BAC851-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{18.38158pt}\def\robExtDepth{12.84158pt}


==> robustExternalize/robExt-D1CAB95DA02DA1243667B17B6EF440FF-out.tex <==
\def\robExtWidth{136.19514pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-D326C82EDB629844CAFB4F892BE37742-out.tex <==
\def\robExtWidth{77.12044pt}\def\robExtHeight{31.59554pt}\def\robExtDepth{26.45557pt}


==> robustExternalize/robExt-D35C524B8F708F487315CB2901718D72-out.tex <==
\def\robExtWidth{83.43303pt}\def\robExtHeight{14.42296pt}\def\robExtDepth{9.28297pt}


==> robustExternalize/robExt-D5D2C0403404A568BFB71901B0BB0ACF-out.tex <==
\def\robExtWidth{88.15164pt}\def\robExtHeight{24.91135pt}\def\robExtDepth{19.77138pt}


==> robustExternalize/robExt-D960A8476EDCE8DFF0DB2A44BE4EAD3E-out.tex <==
\def\robExtWidth{145.14041pt}\def\robExtHeight{17.39125pt}\def\robExtDepth{12.65128pt}


==> robustExternalize/robExt-D9A7E44DD23F32D3FF301D059A456600-out.tex <==
\def\robExtWidth{138.8552pt}\def\robExtHeight{16.65782pt}\def\robExtDepth{11.91782pt}


==> robustExternalize/robExt-DA59C6E8B86E6DD6BB458E789317F6AA-out.tex <==
\def\robExtWidth{148.04405pt}\def\robExtHeight{22.46948pt}\def\robExtDepth{17.32948pt}


==> robustExternalize/robExt-DAE36E0611193C15D55DA00E4B84994D-out.tex <==
\def\robExtWidth{135.64516pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-DB32A1E94652A88301FDC2DB46F1984F-out.tex <==
\def\robExtWidth{169.25131pt}\def\robExtHeight{38.95305pt}\def\robExtDepth{33.81305pt}


==> robustExternalize/robExt-DC2E37E0AE75D18BB514228918AB0447-out.tex <==
\def\robExtWidth{91.24539pt}\def\robExtHeight{40.27585pt}\def\robExtDepth{35.13585pt}


==> robustExternalize/robExt-DCD62734244E036DCDBA1DD376B37F3D-out.tex <==
\def\robExtWidth{106.63252pt}\def\robExtHeight{39.37866pt}\def\robExtDepth{37.17165pt}


==> robustExternalize/robExt-DEA26B9C692085ECC21902D5D4670A28-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{17.98158pt}\def\robExtDepth{13.24158pt}


==> robustExternalize/robExt-DECB44A8701A5C9A32BA5950A9E90DA9-out.tex <==
\def\robExtWidth{136.19514pt}\def\robExtHeight{46.82935pt}\def\robExtDepth{41.68935pt}


==> robustExternalize/robExt-DEDA0CFF4360A15C757DCFE9DD631858-out.tex <==
\def\robExtWidth{260.4775pt}\def\robExtHeight{52.78665pt}\def\robExtDepth{47.64665pt}


==> robustExternalize/robExt-DFFC8BAAC678EE3796328AA393359E16-out.tex <==
\def\robExtWidth{82.15547pt}\def\robExtHeight{21.91309pt}\def\robExtDepth{16.77309pt}


==> robustExternalize/robExt-E0960F631B6F4D4E8B71CFFB0C2326B8-out.tex <==
\def\robExtWidth{142.54558pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-E15B7E2DF927B023A8EFD32BD500AAA9-out.tex <==
\def\robExtWidth{50.71754pt}\def\robExtHeight{17.98158pt}\def\robExtDepth{13.24158pt}


==> robustExternalize/robExt-E1854C3D47039B2315D6F0D88DE2A1CE-out.tex <==
\def\robExtWidth{153.20126pt}\def\robExtHeight{45.65437pt}\def\robExtDepth{40.5144pt}


==> robustExternalize/robExt-E6A6B511D9956E2A274A111380003685-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{27.11975pt}\def\robExtDepth{21.97977pt}


==> robustExternalize/robExt-E843C9B455CCBED2351892F9B1898E28-out.tex <==
\def\robExtWidth{142.54558pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-EA1855450827EDF1F37554E2745507B1-out.tex <==
\def\robExtWidth{34.98367pt}\def\robExtHeight{9.12518pt}\def\robExtDepth{3.9852pt}


==> robustExternalize/robExt-EAC1C9A023ADD6D3F265D1FBFA5AF3E0-out.tex <==
\def\robExtWidth{219.01166pt}\def\robExtHeight{38.95305pt}\def\robExtDepth{33.81305pt}


==> robustExternalize/robExt-EC2A9110C8FDE51DD078768C83F51B84-out.tex <==
\def\robExtWidth{148.44968pt}\def\robExtHeight{18.54439pt}\def\robExtDepth{13.80438pt}


==> robustExternalize/robExt-ECB828AF7660F598264A2FC3E5C36975-out.tex <==
\def\robExtWidth{173.02751pt}\def\robExtHeight{57.57454pt}\def\robExtDepth{52.43456pt}


==> robustExternalize/robExt-ED108D6E564DCD17110C59DE4C179F3E-out.tex <==
\def\robExtWidth{95.64664pt}\def\robExtHeight{28.40558pt}\def\robExtDepth{22.8656pt}


==> robustExternalize/robExt-EDBFBF54F227D7EC434205B00A71395E-out.tex <==
\def\robExtWidth{30.20703pt}\def\robExtHeight{16.65031pt}\def\robExtDepth{11.91034pt}


==> robustExternalize/robExt-EED7A1D455E0172EF85242AC472B318F-out.tex <==
\def\robExtWidth{126.53416pt}\def\robExtHeight{18.54439pt}\def\robExtDepth{13.80438pt}


==> robustExternalize/robExt-F0F9337A269854491B0B2140BA5F4D72-out.tex <==
\def\robExtWidth{107.07126pt}\def\robExtHeight{26.888pt}\def\robExtDepth{21.74803pt}


==> robustExternalize/robExt-F160005C1C28B6F15549C2FFB69CFAA5-out.tex <==
\def\robExtWidth{86.66666pt}\def\robExtHeight{19.05672pt}\def\robExtDepth{13.91672pt}


==> robustExternalize/robExt-F223A4665363BAD3542863F4CD46C80D-out.tex <==
\def\robExtWidth{104.53047pt}\def\robExtHeight{32.74596pt}\def\robExtDepth{27.60597pt}


==> robustExternalize/robExt-F2EEE252BA5313DDCA35BCFBA2DE9898-out.tex <==
\def\robExtWidth{31.53702pt}\def\robExtHeight{20.27449pt}\def\robExtDepth{15.13449pt}


==> robustExternalize/robExt-F2FD8B37497A08FC216FFEEE735BDEA2-out.tex <==
\def\robExtWidth{143.09557pt}\def\robExtHeight{31.8491pt}\def\robExtDepth{26.7091pt}


==> robustExternalize/robExt-F3676D074C2F5351885F255C04574694-out.tex <==
\def\robExtWidth{167.4136pt}\def\robExtHeight{19.4535pt}\def\robExtDepth{14.71353pt}


==> robustExternalize/robExt-F3CA03484842BEB4107214DAD4BCBF96-out.tex <==
\def\robExtWidth{134.00769pt}\def\robExtHeight{31.28891pt}\def\robExtDepth{25.74893pt}


==> robustExternalize/robExt-F4C91576F5324C74C1CEE1D30895EEB3-out.tex <==
\def\robExtWidth{128.68774pt}\def\robExtHeight{21.13821pt}\def\robExtDepth{15.99825pt}


==> robustExternalize/robExt-F603B86671207758C12FB050B9F16B15-out.tex <==
\def\robExtWidth{198.40884pt}\def\robExtHeight{22.41057pt}\def\robExtDepth{17.27057pt}


==> robustExternalize/robExt-F644BE4AC33860AE3A30059FE06C39C0-out.tex <==
\def\robExtWidth{196.3623pt}\def\robExtHeight{28.35309pt}\def\robExtDepth{23.6131pt}


==> robustExternalize/robExt-F680156B6A3DD9411FF99133206E3898-out.tex <==
\def\robExtWidth{197.77689pt}\def\robExtHeight{26.23335pt}\def\robExtDepth{21.09335pt}


==> robustExternalize/robExt-FA6B042493EAA8D8B7F0FA7966C7D4B4-out.tex <==
\def\robExtWidth{135.09517pt}\def\robExtHeight{39.40129pt}\def\robExtDepth{34.2613pt}


==> robustExternalize/robExt-FB223DE606D13C8FB37C504AF0F5AF46-out.tex <==
\def\robExtWidth{254.78696pt}\def\robExtHeight{52.78665pt}\def\robExtDepth{47.64665pt}


==> robustExternalize/robExt-FE64CE25B2F1ABDD4F2770DB535181BE-out.tex <==
\def\robExtWidth{202.05284pt}\def\robExtHeight{28.35309pt}\def\robExtDepth{23.6131pt}

